Product traits, decision-makers, and household low-carbon technology adoptions: moving beyond single empirical studies

Although single empirical studies provide important insights into who adopts a specific LCT for what reason, fundamental questions concerning the relations between decision subject (= who decides), decision object (= what is decided upon) and context (= when and where it is decided) remain unanswered. In this paper, this research gap is addressed by deriving a decision framework for residential decision-making, suggesting that traits of decision subject and object are determinants of financial, environmental, symbolic, normative, effort and technical considerations preceding adoption. Thereafter, the decision framework is initially verified by employing literature on the adoption of photovoltaic systems, energy-efficient appliances and green tariffs. Of the six proposed relations, two could be confirmed (financial and environmental), one could be rejected (effort), and three could neither be confirmed nor rejected due to lacking evidence. Future research on LCT adoption could use the decision framework as a guidepost to establish a more coordinated and integrated approach, ultimately allowing to address fundamental questions.

==> Codes.tex <==
%Figure, depending on [H], [h], [h!] etc, the placement is more or less free
\begin{figure}[H]
\centering
\includegraphics[width=\linewidth, height=\textheight,keepaspectratio]{VBN.png}
\caption{\cite{stern2000new}}
\label{fig_spot}
\end{figure}

%textsizes
	            standard font size
command 	    10pt 	11pt 	12pt
\tiny       	5pt 	6pt 	6pt
\scriptsize 	7pt 	8pt 	8pt
\footnotesize 	8pt 	9pt 	10pt
\small 	        9pt 	10pt 	11pt
\normalsize 	10pt 	11pt 	12pt
\large 	        12pt 	12pt 	14pt
\Large 	        14pt 	14pt 	17pt
\LARGE 	        17pt 	17pt 	20pt
\huge 	        20pt 	20pt 	25pt
\Huge 	        25pt 	25pt 	25pt
%change a word
{\large word}

%nice table, one page, good readability
\begin{table}
\small
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{5pt}
\setcellgapes{1.5pt}\makegapedcells
    \caption{Selected literature for analysis}
    \label{tab: selected literature}
\begin{tabularx}{\linewidth}{XXXXXX}
\toprule
\midrule
\hline
\end{tabularx}
\end{table}


%large table, multiple pages, rotated, header shown on every page, small font size
\begin{landscape}
\small
\begin{longtable}{p{.25\linewidth} p{.42\linewidth} p{.18\linewidth} p{.15\linewidth}}
    \caption{Selected literature for analysis}
    \label{tab: selected literature}
\hline
\textbf{Title} & \textbf{Objective} & \textbf{Survey method} & \textbf{Analysis}\\ 
\hline
\endhead
%....\\
\midrule
\multicolumn{6}{l}{\textbf{LCT traits}}\\ %Zwischenüberschrift
\hline
Initial cost & \multicolumn{2}{l}{The initial financial investment required to adopt} & High & Medium & Low\\ %Zeile mit Spalte 2 und 3 verbunden
\hline
Pay-off period & \multicolumn{2}{l}{\begin{minipage}{.65\linewidth}In the case of a positive long-term financial effect, the pay-off period describes how long it takes for the investment to reach its break-even point\end{minipage}} & High & Low & n.a.\\ %Zeile mit Spalte 2 und 3 verbunden, incl. textbreak wegen langem Textinhalt ({p} geht nicht)
\bottomrule
\end{longtable}
\end{landscape}

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************

